Analyzing Many Simulations of Hybrid Programs in Lince

Hybrid systems are increasingly used in critical applications such as medical devices, infrastructure systems, and autonomous vehicles. Lince is an academic tool for specifying and simulating such systems using a C-like language with differential equations. This paper presents recent experiments that enhance Lince with mechanisms for executing multiple simulation variants and generating histograms that quantify the frequency with which a given property holds. We illustrate our extended Lince using variations of an adaptive cruise control system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{88}
\providecommand{\publicationstatus}{Matt Luckcuck, Maike Schwammberger \& Mengwei Xu (Eds.):\\
Seventh International Workshop on Formal Methods\\
for Autonomous Systems (FMAS 2025)\\
EPTCS 436, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{https://dx.doi.org/10.4204/EPTCS.436.9}{10.4204/EPTCS.436.9}}
\pdfoutput=1

